Geodetic Set on Graphs of Constant Pathwidth and Feedback Vertex Set Number

In the \textsc{Geodetic Set} problem, the input consists of a graph $G$ and a positive integer $k$. The goal is to determine whether there exists a subset $S$ of vertices of size $k$ such that every vertex in the graph is included in a shortest path between two vertices in $S$. Kellerhals and Koana [IPEC 2020; J. Graph Algorithms Appl 2022] proved that the problem is $\W[1]$-hard when parameterized by the pathwidth and the feedback vertex set number of the input graph. They posed the question of whether the problem admits an $\XP$ algorithm when parameterized by the combination of these two parameters. We answer this in negative by proving that the problem remains \NP-hard on graphs of constant pathwidth and feedback vertex set number.

==> np-hardness-treewidth-smd.tex <==
% !TEX root = ./main.tex
\section{Strong Metric Dimension}

A vertex $s \in V(G)$ \emph{strongly resolves} a pair of vertices
$u,v \in V(G)$ if there exists a shortest path from 
$u$ to $s$ containing $v$, or a shortest path from $v$ to 
$s$ containing $u$. 
A subset $S \subseteq V(G)$ is a \emph{strong resolving set} 
is every pair of vertices in $V(G)$ is strongly 
resolved by a vertex in $S$.

To this end, we present a reduction from 
\textsc{Exact-$3$-Partitioned-$3$-SAT} (see \Cref{sec:preliminaries})
to \textsc{Strong Metric Dimension}.
We use the relation
between \textsc{Strong Metric Dimension}
and the \textsc{Vertex Cover} problem,
which was established in~\cite{OP07},
to prove the theorem.
We need the following definition in order
to state the relationship.
\begin{definition}
\label{def:mutually-max-distant}
Given a graph $G$, we say a vertex $u\in V(G)$ is maximally distant from $v\in V(G)$ if
there is no $x \in V(G) \setminus \{u\}$ such that a shortest path between $x$ and $v$ contains $u$.
Formally, for every 
$y \in N(u)$, we have
$d(y, v) \le d(u, v)$.
If $u$ is maximally distant from $v$, and
$v$ is maximally distant from $u$, 
then $u$ and $v$ are \emph{mutually maximally 
distant} in $G$, and we write $u \bowtie v$.
\end{definition}
For any two mutually maximally distant
vertices in $G$, there is no vertex in $G$ 
that strongly resolves them, except themselves. 
Hence, if $u \bowtie v$ in $G$, 
then, for any strong resolving set $S$ of 
$G$, at least one of $u$ or $v$ is in $S$,
i.e., $|\{u, v\}\cap S|\geq 1$.
Oellermann and Peters-Fransen~\cite{OP07}
showed that
this necessary condition
is also sufficient.
Consider an auxiliary graph $G_{SR}$
of $G$ defined as follows.
\begin{definition}
\label{def:strong-resolving-graph}
Given a connected graph $G$, the 
\emph{strong resolving graph} of $G$, 
denoted by $G_{SR}$, has vertex set 
$V(G)$ and two vertices $u, v$ are adjacent
if and only if
$u$ and $v$ are mutually maximally 
distant in $G$, i.e., $u \bowtie v$.
\end{definition}
%Oellermann and Peters-Fransen proved that the 
%problem of finding the strong metric dimension 
%of $G$ is equivalent to 
%the problem finding the minimum vertex cover 
%$G_{SR}$.
\begin{proposition}[Theorem 2.1 in \cite{OP07}]
\label{prop:strong-met-dim-equiv-vc}
For a connected graph $G$,
$\smd(G) = \vc(G_{SR})$.
\end{proposition}
In light of the above proposition,
it is sufficient to prove the following lemma.
\begin{lemma}
\label{lemma:SAT-SMD-VC}
There is a polynomial-time reduction that,
given an instance $\psi$ of 
\textsc{Exact-$3$-Partitioned-$3$-SAT} 
on $3n$ variables,
returns an equivalent instance
$(G, k)$ of \textsc{Strong Metric Dimension}
such that 
$\vc(G) = \calO(\log(n))$
and $\vc(G_{SR}) = k$.
\end{lemma}

Recall the textbook reduction from
\textsc{$3$-SAT} to \textsc{Vertex Cover}
\cite{DBLP:books/daglib/0015106}.
In this, we add matching edges corresponding 
to variables, and vertex-disjoint triangles
corresponding to clauses.
Finally, we add edges between two vertices
corresponding to the same literal 
on 
the ``variable-side'' and the ``clause-side''.
We adopt the same reduction for
\textsc{Exact-$3$-Partitioned $3$-SAT} to 
\textsc{Vertex Cover}.

\begin{figure}[h]
\begin{center}
%\includegraphics[scale=0.65, trim={0cm 4.5cm 0 3.3cm}, clip]{./images1/3-Par-3-SAT-to-VC.pdf}
\includegraphics[scale=0.9]{./images/overview.pdf}
\end{center}
\caption{
Overview of the reduction from
\textsc{Exact-$3$-Partitioned-$3$-SAT} to
\textsc{Vertex Cover}.
In Step~\ref{step:add-ind-set}, we add
all the independent sets mentioned.
In Step~\ref{step:add-variable-edges}, we
add matching green edges corresponding
to the assignment of the variables.
In Step~\ref{step:add-clause-edges},
we add purple triangles 
corresponding to clauses.
For example, the {purple} 
triangle corresponds to the 
clause $(x^{\alpha}_{3} \lor \neg x^{\beta}_2
\lor x^{\gamma}_{1})$.
In Step~\ref{step:add-variable-clause-edges},
we add red edges connecting the vertices
corresponding to the same literal
on the ``variable-side'' and ``clause-side''.
\label{fig:3-Par-3-SAT-to-VC}}
\end{figure}

Given an 
instance $\psi$ of 
\textsc{Exact-3-Partitioned-3-SAT},
with $m$ clauses and $3n$ variables
partitioned equally into $X^{\alpha}, X^{\beta}, X^{\gamma}$,
we construct the graph $H$ as follows.
\begin{enumerate}
\item \label{step:add-ind-set}
We rename the variables in $X^{\alpha}$
to $x^{\alpha}_{i}$ for $i \in [n]$. Analogously, we do this
for $X^{\beta}$ and $X^{\gamma}$.
For every $x^{\alpha}_i$,
we add two vertices $x^{\alpha}_{i, t}$
and $x^{\alpha}_{i, f}$
for the positive and negative literal, respectively.
Define $X^{\alpha}_{T}$ and $X^{\alpha}_{F}$
as the collection of vertices 
corresponding to the positive and negative 
literals of the variables
in $X^{\alpha}$, respectively.
We define the sets 
$X^{\beta}_{T}, X^{\beta}_F, X^{\gamma}_T,$
and $X^{\gamma}_F$, similarly.
%All these sets are independent sets.

Consider a clause $C_q = (x^{\alpha}_i \lor
\neg x^{\beta}_j \lor x^{\gamma}_{\ell})$.
We add three vertices: $x^{\alpha, q}_{i, t}$, 
$x^{\beta, q}_{j, f}$, and 
$x^{\gamma, q}_{\ell, t}$,
and the edges to make it a triangle.
Let $U^{\alpha}_T$ be the collection
of vertices corresponding to the 
positive literals of
variables in $X^{\alpha}$.
Formally, $U^{\alpha}_T = \{x^{\alpha, q}_{i, t} \mid$ 
there is a clause $C_q$
that contains the positive literal of the variable $x^{\alpha}_i\}$.
Note that, for a variable $x^{\alpha}_i$,
there may be multiple vertices corresponding 
to its positive literal in $U^{\alpha}_T$ depending on the number of clauses that contain $x^{\alpha}_i$.
We analogously define $U^{\alpha}_F$,
$U^{\beta}_T$, $U^{\beta}_F$, $U^{\gamma}_T$, and $U^{\gamma}_F$.
See \cref{fig:3-Par-3-SAT-to-VC}
for an illustration.


\item 
\label{step:add-variable-edges}
We add matching edges across 
$X^{\alpha}_T$ and $X^{\alpha}_F$
connecting $x^{\alpha}_{i, t}$
and $x^{\alpha}_{i, f}$ for every $i \in [n]$.
We add similar matching edges across
$X^{\beta}_T$ and $X^{\beta}_F$, and
$X^{\gamma}_T$ and $X^{\gamma}_F$. 
See the {green} edges in \cref{fig:3-Par-3-SAT-to-VC}.

\item 
\label{step:add-clause-edges}
As $\psi$ is an instance of 
\textsc{Exact-$3$-Partitioned-$3$-SAT}, 
for any clause there is a triangle that
contains {exactly} one vertex from each of
$U^{\alpha}_T \cup U^{\alpha}_F$,
$U^{\beta}_T \cup U^{\beta}_F$, and
$U^{\gamma}_T \cup U^{\gamma}_F$.
%Recall that, as we are dealing with \textsc{Exact-$3$-Partitioned-$3$-SAT}, every clause contains exactly $3$ variables.
See the purple triangle in \cref{fig:3-Par-3-SAT-to-VC}.
For each clause, we add the edges to form its
corresponding triangle.

\item
\label{step:add-variable-clause-edges}
Finally, we add edges connecting 
a vertex corresponding to a literal on the
variable-side to vertices corresponding
to the same literal on the clause-side.
See the red edges in \cref{fig:3-Par-3-SAT-to-VC}.
\end{enumerate}

The reduction returns $(H, k)$ as the 
reduced instance of \textsc{Vertex Cover}, where $k = 3n + 2m$.
The correctness of the following 
lemma is spelled out in \cite{DBLP:books/daglib/0015106}.
\begin{lemma}
\label{lemma:Ex-3-Par-3-SAT-to-VC}
The formula $\psi$, with $3n$ variables and $m$ clauses, is a satisfiable 
\textsc{Exact-3-Partitioned-3-SAT} formula
if and only if $H$ admits a vertex cover
of size $k = 3n + 2m$.
\end{lemma}



In what remains of this section,
our objective is to construct $G$ such that
$G_{SR}$ is as ``close'' to $H$ as possible.
It will be helpful to think about $V(H)$ as a subset of $V(G) = V(G_{SR})$.
We want to construct $G$ such that
all the edges in $E(H)$ are present
in $G_{SR}$, while no undesirable edge 
appears in $G_{SR}$.
We use a \emph{set representation gadget}
and a \emph{bit representation gadget}
for the first and the second part, respectively.
However, for the second part, we need another trick since we may have some undesirable edges.
We ensure that all the edges in
$E(G_{SR}) \setminus E(H)$, i.e.,
undesirable edges, are 
incident to a clique, say $Z$, in $G_{SR}$.
Moreover, there is a vertex $z$ in $Z$ 
such that $N[z] = Z$, i.e., $z$ is not
adjacent to any vertex in $V(G_{SR}) \setminus Z$.
Then, without loss of generality,
we can assume that any vertex cover 
of $G_{SR}$ contains $Z \setminus \{z\}$.  
Hence, all the undesired edges are deleted 
by a pre-processing step while finding
the vertex cover of $G_{SR}$.
In other words, $E(H) = E(G_{SR} - (Z \setminus \{z\}))$. 
This ensures that  
the difficulty of finding a strong resolving
set in $G$ is encoded in finding a vertex cover in $G_{SR} - Z$, a graph with only 
desired edges.
We note the following easy observation
before presenting the primary tools used in 
the reduction.
\begin{observation}
\label{obs:pendant-in-G-to-clique-in-GSR}
Consider a connected graph $G$ that has
at least $3$ vertices.
Suppose $Z \subseteq V(G)$ is the collection
of all the pendent vertices in $G$.
Then, 
$Z$ is a clique in $G_{SR}$, and
every vertex in $N(Z)$ is an isolated
vertex in $G_{SR}$.
\end{observation}
\begin{proof}
Consider any two vertices $z_1, z_2$ in $Z$, and let $u_2$ be the unique neighbor of $z_2$.
It is easy to see that $d(z_1, u_2) < d(z_1, z_2)$.
Hence, $z_2$ is maximally distant from $z_1$.
Using the symmetric arguments, $z_1$ is 
maximally distant from $z_2$, and hence,
$z_1 \bowtie z_2$.
By the construction of $G_{SR}$, there is 
an edge with endpoints $z_1, z_2$.
As these were two arbitrary points in $Z$, we have that
$Z$ is a clique in $G_{SR}$.

Consider an arbitrary vertex 
$v \in V(G) \setminus \{u_2\}$.
If $v \neq z_2$, then $d(v, z_2) > d(v, u_2)$ 
and hence, $u_2$ is \emph{not} maximally distant 
from $v$.
This implies that $u_2$ is not adjacent with
any vertex in $V(G_{SR}) \setminus \{z_2\}$
in $G_{SR}$.
As $G$ is connected and has at least three 
vertices, $u_2$ is not maximally distant from 
$z_2$ either.
Hence, $u_2$ is an isolated vertex in 
$G_{SR}$.
Since $u_2$ is an arbitrary vertex in $N(Z)$, 
the second part of the claim follows.
\end{proof} 


